Interpenetrating Cooperative Localization in Dynamic Connected Vehicle Networks

In this paper, we proposed the Interpenetrating Cooperative Localization (ICL) method to enhance the localization accuracy in dynamic connected vehicle networks. This mechanism makes the information from one group of connected vehicles interpenetrate to other groups without full communication between all nodes, thus improving the utility of information in a low connected vehicle penetration situation. We tested the approach using the dynamic traffic data collected in the Safety Pilot Model Deployment program in Ann Arbor Michigan, USA, with dynamic changing networks due to the traveling of vehicles and packet drops of the Dedicated Short-Range Communication. Results show enhancement of localization accuracy with errors reduced by up to 70 % even in complex dynamic scenarios.

==> 1.tex <==
\textbf{Note} The trajectories contain various urban driving acts. Each vehicle may conduct a term of straight-driving, then do turns or U-turns, and may short stops in between (such as stop at the red traffic light). It is interesting that in a few cases during simulations, the positioning errors for the host vehicle during its brief stop period were observe to increase, followed by a decrease after it starts moving again. It's not yet clear whether such incidents are due to coincidence or have fundamental reasons behind.

The position data used for this work are from real-world vehicle dataset, which imitate the actual traffic scenarios where all vehicles moving on the real city-roads start synchronously from different position and changing velocities following actual roads, but estimated under the same group of satellites. 
Also, to select the optimal group of vehicles to form network configuration, 
%a Branch and Bound algorithm and
 a Cross Entropy (CE) method is implemented, 
 %the first under
given the assumption that the GNSS non-common errors for each vehicle members are roughly the same
%, and the second assumes the GNSS non-common errors to 
would be different in the large scale dynamic traffic.
The practical packet losses in the connect vehicle network regarding Dedicated Short-Range Communication (DSRC) is also implemented, and an analysis is conducted on whether it is workable to reduce the positioning error by rearranging particle weights from different neighboring vehicles.





% \EndWhile
% \State Check if distance from host to vehicle $i$ is within ER %(max range).
% \While{True}
% accept packet from this vehicle
% \EndWhile
% \While{False}
% check if $r(i,k) \le p$
% \While{True}
% accept the packet from this vehicle
% \EndWhile
% \While{False}
% drop this packet
% \EndWhile
% \EndWhile
% \State Check if stackled particles are from neighbors within ER %(effective range)
% \While{True}
% give higher resample weights;
% \EndWhile
% \While{False}
% give lower resample weights;
% \EndWhile
% \If
% \EndIf
%\Comment{The gcd is b}

% \begin{table}[ht]
% \caption{Multi-row table}
% \begin{center}
% \begin{tabular}{cc}
%     \hline
%     \multirow{3}{*}{Multirow}& Net $N_1$ \\&Net $N_2$\\&Net $N_3$\\
%     \hline
% \end{tabular}
% \end{center}
% \label{tab:multicol}
% \end{table}

%  \begin{figure}[ht]
% \includegraphics[width=\linewidth]{fig/RBPF_Np_75_Ns_80_error.png}
%  	\caption{localization error w/ RBPF vs error w/o RBPF}
%  	\label{fig:stn_vehi_err}
%  \end{figure}
 
% The simulation results for... are presented in Fig. \ref{fig:dist_vehi_xy}, where...

 % (1) Without Packet drops
% \begin{figure}[ht]
% \includegraphics[width=\linewidth]{fig/RBPF_dyn_all_veh_better_Ns_200_act_filt_noisy_xy.png}
%  	\caption{localization error w/ RBPF vs error w/o RBPF}
%  	\label{fig:stn_vehi_xy}
%  \end{figure}
%  \begin{figure}[ht]
% \includegraphics[width=\linewidth]{fig/RBPF_dyn_all_veh_better_Ns_200_error.png}
%  	\caption{localization error w/ RBPF vs error w/o RBPF}
%  	\label{fig:dyn_vehi_err}
%  \end{figure}
%  (2) With Packet drops according to DSRC Range
%  \item 
% \subsection{Performance under full dynamic situations}

% \begin{figure}[ht]
% \includegraphics[width=\linewidth]{fig/pkt_drp_distrb.png}
%  	\caption{Packet loss for vehicles from host further away from DSRC range, and vehicles given higher weights who are within ER. This is for a 50 vehicle network.}
%  	\label{fig:pkt_drp_distb}
%  \end{figure}

% \begin{figure}[ht]
% \includegraphics[width=\linewidth]{fig/RBPF_Np_75_Ns_80_act_flt_noisy_xy.png}
%  	\caption{Stationary case: localization error w/ RBPF vs error w/o RBPF}
%  	\label{fig:dist_vehi_xy}
%  \end{figure}

% The connection structure for a 24 vehicle network is shown as in Fig. \ref{fig:24vehiDistb}, for a 38 vehicle network as in \ref{fig:38vehiDistb}, for a 50 vehicle network as in \ref{fig:50vehiDistb}. 

% \subsection{Optimize the Vehicle Network Configuration}
% Intuitively, in order to produce a good estimation of the
% common error, the road constraints should be rich enough
% so that common error in different directions can be detected.
% This richness is expected to be enhanced with the number of
% vehicles and the diversity of the road directions.
% As was studied in our previous work \cite{DBLP:journals/corr/ShenZS17a}, to optimally select a group of $ M(M \leq N) $ vehicles out
% of the total $N$ available connected vehicles to implement CMM, we can use Branch and Bound (B$\&$B) method if the variances are similar for each vehicle such as on the high way, and use
% Cross Entropy (CE) method if the difference of variances are not trivial, such as in the urban situations. 
% The B$\&$B method
% is expected to find a near optimal, but is only valid under assumption that 
% %solution as long as 
% the
% variances are approximately the same.
% %, under the assumption that all the vehicle members are under equal non-common error variance situations. 
% Intuitive, however, non-common error variance for vehicles vary in the large scale urban dynamic scenario.
% % the B$\&$B method 
% %is applied to the case where all the vehicles have the same non-common error variance. Although it is rare, in practice, to have exactly same non-common error variance for all the connected vehicles, 
% % \subsubsection{Cross Entropy Method for Network Optimization}
% We thus choose to apply Cross Entropy Method instead, which can be used for network optimization under variant non-common error variance situations, where road angles as random variables
% drawn from some distribution. The square error becomes a
% random variable as a function of the road angles as well as the
% non-common error variances. It will be proved that in the limit
% that the number of vehicles goes to infinity, the expectation of
% the geometric error $e_0^2$
% is minimized if the angles of the roads
% on which the vehicles travel obey a uniform distribution.

% (Choices:

% Study the select $C_{50}^{24}$ -- might mot show difference due to small sample set.

% Or study the select $C_{1000}^{50}$. Need new data.)

% \section{Formulation of Decentralized Network}

% \subsection{Notations}

% which is calculated by averaging the estimations of $i$'s common error from all neighboring vehicles $j \in E$ over the particles.



% \begin{algorithm}
% \caption{Packet loss and weight arrangement}\label{alg:pkt_loss}
% \begin{algorithmic}[1]
% \Procedure{DSRC weight}{Dist}
% %\Comment{The g.c.d. of a and b}
% \State Assign a label $ r(i,k)$  to $i$th vehicle at timestep $k$, $ r(i,k) \in [0,1]$;
% \State Set a accept probability $ p = PDR$
% %, i.e, $p_{CR} = 0.7$, $p_{MR} = 0.1$;
% \State Calculate distance from $i$th vehicle to the host vehicle at timestep $k$, record as $D_k^i$
% % \State Calculate particle weights and update $X_t$
% \State At timestep k, check if $D_k^i \le$ ER
% \While{True}
% check if $r(i,k) \le p_{ER}$
% \While{True}
% Accept packet and stack into particle
% \EndWhile
% \While{False}
% Check if $D_k^i \le MR$
% \While{True}
% check if $r(i,k) \le p_{D_{k}^i}$
% \While{True}
% Accept packet and stack into particle 
% %(with lower resample weight, i.e., times a coefficient $\le 1$)
% \EndWhile
% \While{False}
% Drop this packet
% \EndWhile
% \EndWhile
% \While{False}
% Drop this packet
% \EndWhile
% \EndWhile
% \EndWhile
% \While{False}
% Drop this packet
% \EndWhile
% \State Normalize the sum of weights for one set of particles to 1;
% \EndProcedure
% \end{algorithmic}
% \end{algorithm}

% \textbf{note} Dynamic trajectory plots in 3d (time-x-y) and t-x, ty are not presented here.
%    \begin{figure}[ht]
% \includegraphics[width=\linewidth]{fig/RBPF_RW_50veh_501-1500_tx.png}
%      \caption{50 vehicle network from Safety Pilot: timesteps and east position as x-y axis}
%      \label{fig:rw_50_vehi_tx}
%  \end{figure}

%  \begin{figure}[ht]
% \includegraphics[width=\linewidth]{fig/RBPF_RW_50veh_501-1500_3d.png}
%      \caption{50 vehicle network from Safety Pilot: timestep ($\Delta$ t = 0.1s) -north-east as axis; orange line for actual postions, blue line for RBPF filtered positions (Red dot is the start (at 501th timestep) and black dot is the end (at 1500th timestep), black line stands for the direct GNSS estimated position without applying RBPF}
%      \label{fig:rw_50_vehi_3d}
%  \end{figure}
 
%     \begin{figure}[ht]
% \includegraphics[width=\linewidth]{fig/RBPF_RW_50veh_501-1500_ty.png}
%      \caption{50 vehicle network from Safety Pilot: timesteps and north position as x-y axis}
%      \label{fig:rw_50_vehi_ty}
%  \end{figure}
 
% \end{enumerate}

==> paper_backup.tex <==
\section{Introduction}

Connected vehicle technologies  use crude GNSS measurements from a group
of connected vehicles and match their locations to a digital
map, which provide
an efficient approach for enhancing the localization accuracy. A Global Navigation Satellite System
(GNSS) receiver calculates its position from pseudo-range
measurements of multiple satellites. Pseudo-ranges contain
error which can be decomposed into common error (due to
satellite clock error, ionospheric and tropospheric delays) and
non-common error (due to receiver noise, receiver clock error
and multipath error). The nominal accuracy of pseudo-ranges
for a single-band receiver is about 10 to 20 meters, which
results in a position error of several meters [1]. Without further
improvement, this crude GNSS error is too large for many
safety functions as the lane of vehicles cannot be robustly.


An alternative to improving
GNSS absolute positioning without incurring infrastructure
costs is cooperative map matching (CMM). Assuming that
most vehicles travel within lanes, the correction to the common
localization biases can be determined so that the corrected
positions of a group of vehicles best fit the map. In this work, we presented a practical study is
presented that aims at applying a framework for quantitatively
evaluating effects of the road constraints on the CMM accuracy
and for eventual optimization of the CMM network. A localization method was proposed based on the optimized configuration of vehicle connections, and applied RBPF approach for a empirical localization scenario considering a Dedicated Short Range Communication (DSRC) of packet-drops varying on vehicle distances, upon this network structure produced an improved CMM error reduction. A Rao-Blackwellized particle filter (RBPF) is then used to
jointly estimate the common biases of the pseudo-ranges and
the vehicle positions \cite{zhao2017accelerated}.
While further error reduction is expected by
increasing the number of participating vehicles, fundamental
questions on how the vehicle membership of the cooperative map matching (CMM) affects
the performance of the GNSS-based localization results is crucial for design and optimization
of the vehicle network. The quantitative relationship between the
estimation error and the road constraints which has also been systematically
investigated to provide insights.

%In this paper. A Branch and Bound algorithm and a Cross Entropy method are developed to minimize this error by selecting the optimal group of vehicles. Two types of the GNSS error distributions were tested, the first with equal non-common error variance and the second with variant non-common error variance. 

% \begin{figure}[h]
% 	\centering
% 	\includegraphics[width=\linewidth]{fig/cute-frog-umbrella-rain.jpg}
% 	\caption{How frog survive in a rain}
% 	\label{fig:frog}
% \end{figure}

\section{OPTIMIZING THE SELECTION OF VEHICLES}

Combine the optimization of vehicle connection with RBPF under dynamic situations. 

To optimally select a group of $ M(M \leq N) $ vehicles out
of the total $N$ available connected vehicles to implement CMM, using use Branch and Bound (B\&B) method if the variances are similar for each vehicle such as on the high way, and using
Cross Entropy (CE) method if the difference of variances are not trivial, such as in the urban situations. 

\subsection{Selection of Vehicle Connections}

Due to the limits of empirical DSRC, we need to form a optimal selection of vehicles to be connected, considering the limit of communication bandwidth and ratio of packet drops under dynamic scenario, where each vehicle move along the road with a reasonable speed.

\subsubsection{Branch and Bound Method for Network Optimization}

Assumue under equal non-common error variance situations,
the B\&B method is applied to the case where all the
vehicles have the same non-common error variance. Although
it is rare, in practice, to have exactly same non-common error
variance for all the connected vehicles, the B\&B method
is expected to find a near optimal solution as long as the
variances are approximately the same.

\subsubsection{Cross Entropy Method for Network Optimization}

Under variant non-common error variance situations.

\subsection{Packet Drop Distribution}

We assume a sigmoid distribution of packet drop regarding the distance between connected vehicles, according to the DSRC Range.


\subsubsection{DSRC Range}

With the deployment of Dedicated Short Range Communications
(DSRC) technique in the real world, connected
vehicles provide an alternative for improving localization error
by correcting common localization error of multiple GNSS
receivers installed on multiple vehicles. 

To characterize the performance of DSRC, the following metrics are defined:

(related)


% (1) Packet Delivery Ratio (PDR): the ratio of successful communication events to the total number of transmission attempts at a given distance between two DSRC units.

% (2) Maximum Range (MR): the maximum distance at which the vehicle or road side equipment (RSE) can receive packets from another vehicle with a larger-than-zero packet delivery ratio.

% (3) Effective Range (ER): the distance within which the vehicle or RSE can receive packets from other vehicles with a packet delivery ratio larger than a defined threshold (e.g., $50\%$).

% Alam et al. [13] developed a cooperative positioning method that improves the relative positioning between two vehicles by fusing the shared pseudo-range observations. The relative positioning
%accuracy of this method outperforms that of DGNSS alone.
%Wang [14] proposed an augment DGPS that tightly integrated
%DGPS, range and bearing observations in a small network of
%vehicles or infrastructure points, which outperforms the DGPS
%in terms of absolute positiong.

\subsubsection{Previous used model}

(Method description copied from Previous presentation slides: need to edit) 
Adjust resample weights according to packet drop range of distance:

(i) At each time step k, assign label as a random number $ lb(i,k) \in [0,1]$ to all packets from the i-th neighboring vehicles, $i \in \{1,2,..., Nv\}$, $ k \in \{1,2,...,Ns\} $;

(ii) Set a block probability $ p $, i.e, p = 0.3;

(iii) Check if distance from host to vehicle I is within confidence range.
If true, use the packet and go to RBPF;
If false, check if 'label(i,Ns) $\ge$ block prob': if true, accept the packet and go to RBPF process;
if false, drop this packet.

(iv) Check if particles are from “close” neighbors in resample process:
if true, give higher resample weights;
if false, give lower resample weights;

(v) Normalize the distribution and make sure that the weights for one set of particles add up to 1;

\section{DYNAMIC VEHICLE NETWORK FORMULATIONS}
% Combine the dynamic scenario

Three types of dynamic model was simulated. 
The first model assumed a straight-heading situation, given that every vehicle within the network would drive on a straight-line (i.e., driving along the highway), each with a different but constant velocity within the legal range, and along their own directions predetermined by the associated road-map angles. 
The second model assumed that the host vehicle moving around an ellipse circuit (semi-axi a = 160m, semi-axi b = 80m), given that all the neighboring vehicles moving each in straight line with their own constant velocity, as presented in the first model.

The third model is to implement real-world driving data from the Safety-Pilot dataset, which simulated based on the past 3 years driving data of Ann Arbor city to provide the most representative corresponding routes for 24,38, 50 vehicle networks according to actual road conditions. Trajectories are randomly selected from the 100k record
trajectories from the database, based on the central point of the smallest rectangle which can encompass the trajectory. This provide a method which gave the trajectories in area with tense traffic flows to have higher probability to be chosen, where number of vehicles and simulation 
duration are the two inputs. 

\subsection{Straight Heading with Constant Velocities}

In this case, we provide...

\subsection{Host Vehicle Traversing in Ellipse}

In this case, we provide...

\subsection{Real-World Dynamic Trajectories}

In this case, we provide...

\section{RBPF regardng road constrains}

We used a particle filter to implement our method as follow.
First, the target vehicle initiates 75 particles according to
its prior position estimation, which is in this case the GPS
measured position. The next step is to update the weights of
the particles with respect to the road constraints. With the
given assumption of negligible non-common error, we can first
set the weights of the particles falling out of the constraints
to zero and then normalize the remaining particle weights in
each iteration of the filter. We apply the road constraints of
each communicating vehicle transformed for the target vehicle
to the initiated particles. Fig. 3 summarizes the particle
filter steps and Fig. 4 illustrates an example of the particle
filter implementation. Finally, the result of the particle filter
is approximated by a Gaussian distribution to calculate the
mean and the covariance matrix of the position estimation.



\section{CMM LOCALIZATION ERROR}
% Combine the dynamic scenario

In our previous work which was presented at the conference
[17], the problem of inferring the true vehicle positions, as
well as the GNSS common biases from the pseudo-range
measurements from a group of vehicles, is addressed by a
Bayesian filtering approach. The aforementioned difficulties
are solved by jointly estimating the common biases and vehicle
positions using a Rao-Blackwellized particle filter (RBPF).

In the RBPF, the correlation between common biases and
vehicle positions is modeled implicitly through the diversity
of the particles. As a result, there is no need for explicit
data fusion. The effect of the multipath biases is mitigated
through a detection-rejection method based on a statistical
test. The particle filter structure allows multiple hypotheses
with respect to the detection of multipath biases, thus making
the detection more robust. In addition, the particle filter is
flexible enough to handle road constraints in a straightforward
manner by manipulating the particle weights according to the
road constraints. It also fully exploits the temporal correlation
through a prediction-update process, eliminating impossible
configurations in the joint space of common biases and vehicle
state variables, drastically reducing the estimation variance.
The computational complexity varies linearly with the number
of vehicles, which makes the proposed RBPF both effective
and efficient.

This paper expands the initial results from the conference
paper. More specifically, the performance of the algorithm
in ... environments with signal blockage is shown
through simulations based on ...

\section{Conclusion}
The conclusion goes here.

1. Introduction of CMM.

2. Problem of CMM and what we've done and remaining issues (i.e., dynamic not considered)

3. Select of optimal choice of vehicle, (mac)

4. How setup communication enviorn
(if everything connected - good, packet drop - bad, proposing another method (penetration)

5. Implementation: collect data from real world road conditions, RBPF for dynamic situation

Introduction:
1. 新闻 (cv : 现实）
2. GPS, 精度重要（cv 基础）
已有：贵；cv与localization 交叉提升；
CMM新方法 （3/4）
, Rohanis, CV give localization increse: how we did; 
3. question limitations;
(old: therotical:
1. car too many?
2. too far? -> interpaenit
3. not evaluracte in RW; not considered packet loss)

4.结构；）

RW: with 1st section
1. how the other people did to improve ll; how we did with CMM;

II. interpenetration cooperation
1. cooperative Local : CMM
2. interpentrating （概念，结构方法）
3. structure 
（图：算法结构流程
接受信号 -》 判断掉包 -》选车 -》CMM -》发出去和其他人fuse）

III. 合于interpanit

IV. Real world unperfectness
GPS error, DSRC, drop, dynamic

V. Simulation
city vehicle model, how SPMD data is used (use graph macheng's sensi 9)

1. 静态
2. 动态

packet drop rate rading
前言，结论

VI. results
VII. Discussion
